Bayesian Optimization for Ion Beam Centroid Correction

An activity of the TRIUMF automatic beam tuning program, the Bayesian optimization for Ion Steering, BOIS, method has been developed to perform corrective centroid steering of beams at the TRIUMF ISAC facility. BOIS exclusively controls the steerers for centroid correction after the transverse optics have been set according to theory. The method is fully online, easy to deploy, and has been tested in low energy and postaccelerated beams at ISAC, achieving results comparable to human operators. scaleBOIS and boundBOIS are naive proof of concept solutions to preferably select beam paths with minimal steering. Repeatable and robust automated steering reduces reliance on operator expertise and operational overhead, ensuring reliable beam delivery to the experiments and thereby supporting TRIUMF's scientific mission.

==> acronyms.tex <==


\DeclareAcronym{BO}{
  short=BO,
  long=Bayesian optimization,
}


\DeclareAcronym{BOIS}{
  short=\texttt{BOIS},
  long=Bayesian Optimization for Ion Steering,
}

\DeclareAcronym{ISAC}{
  short=ISAC,
  long=Isotope Separator and Accelerator,
}

\DeclareAcronym{TRIUMF}{
  short = TRIUMF,
  long  = Canada's National Laboratory for Particle and Nuclear Physics,
}

\DeclareAcronym{ML}{
  short = ML,
  long  = machine learning
}

\DeclareAcronym{GP}{
  short = GP,
  long  = Gaussian process
}
\DeclareAcronym{fc}{
  short = FC,
  long  = Faraday cup
}
\DeclareAcronym{RPM}{
  short = RPM,
  long  = Rotatory Profile Monitor
}
\DeclareAcronym{LPM}{
  short = LPM,
  long  = Linear Profile Monitor
}
\DeclareAcronym{OLIS}{
  short = OLIS,
  long  = Offline Ion Source
}
\DeclareAcronym{RL}{
  short = RL,
  long  = Reinforcement Learning
}
\DeclareAcronym{DRL}{
  short = DRL,
  long  = Deep Reinforcement Learning
}

\DeclareAcronym{HLA}{
  short = HLA,
  long = High Level Applications
}

\DeclareAcronym{NN}{
  short = NN,
  long = Neural Networks
}

\DeclareAcronym{MTBO}{
  short = MT-BO,
  long = Multi-task Bayesian Optimization
}

\DeclareAcronym{AF}{
  short = AF,
  long = acquisition function
}

\DeclareAcronym{RIB}{
  short = RIB,
  long = Rare Isotobe Beams
}

\DeclareAcronym{UCB}{
  short = UCB,
  long = Upper Confidence Bound
}

\DeclareAcronym{EI}{
  short = EI,
  long = Expected Improvement
}



==> packages.tex <==

\usepackage{adjustbox}

\usepackage{dcolumn}% Align table columns on decimal point
\usepackage{bm}% bold math



\bibliographystyle{stuff_notouchy/aip}

\usepackage[utf8]{inputenc}
\usepackage[T1]{fontenc}
\usepackage{mathptmx}
\usepackage{etoolbox}
\usepackage[version=4]{mhchem}
\usepackage{amsmath}
\usepackage{mathrsfs}
\usepackage{multirow}
\usepackage{tabularx}
%\usepackage{natbib}
\usepackage{placeins}
\usepackage{float}
% \usepackage{caption}
% \captionsetup{justification=justified}
\usepackage{subcaption}
% \usepackage{caption}
\usepackage{soul}
% \captionsetup{justification=justified}
\usepackage{acro}

\usepackage[normalem]{ulem}


\usepackage{tikz}
\usetikzlibrary{shapes.geometric, arrows, arrows.meta, positioning, fit}

\DeclareMathAlphabet{\mathcal}{OMS}{cmsy}{m}{n}

\newcommand{\argmax}[1]{\underset{#1}{\operatorname{\text{arg}}\,\operatorname{\text{max}}}\;}
%\input{namestack}

\usepackage{caption}
\captionsetup{justification=raggedright, singlelinecheck=on}


\newcommand{\orcidicon}{\includegraphics[width=8pt]{stuff_notouchy/ORCID-iD_icon-128x128.png}}
\newcommand{\orcidauthor}[1]{%
    \href{https://orcid.org/#1}{\orcidicon}%
}


\usepackage{hyperref}

\hypersetup{
  colorlinks   = true, %Colours links 
  urlcolor     = blue, %Colour for external 
  linkcolor    = black, %Colour of internal links
  citecolor   = red %Colour of citations
}


